Backpropagation-Free 4D Continuous Ant-Based Neural Topology Search

Continuous Ant-based Topology Search (CANTS) is a previously introduced novel nature-inspired neural architecture search (NAS) algorithm that is based on ant colony optimization (ACO). CANTS utilizes a continuous search space to indirectly-encode a neural architecture search space. Synthetic ant agents explore CANTS' continuous search space based on the density and distribution of pheromones, strongly inspired by how ants move in the real world. This continuous search space allows CANTS to automate the design of artificial neural networks (ANNs) of any size, removing a key limitation inherent to many current NAS algorithms that must operate within structures of a size that is predetermined by the user. This work expands CANTS by adding a fourth dimension to its search space representing potential neural synaptic weights. Adding this extra dimension allows CANTS agents to optimize both the architecture as well as the weights of an ANN without applying backpropagation (BP), which leads to a significant reduction in the time consumed in the optimization process: at least an average of 96% less time consumption with very competitive optimization performance, if not better. The experiments of this study - using real-world data - demonstrate that the BP-Free CANTS algorithm exhibits highly competitive performance compared to both CANTS and ANTS while requiring significantly less operation time.

==> sections/001-org_introduction.tex <==
\section{Introduction}
\label{sec:introduction}

Manually optimizing artificial neural network (ANN) structures has been an obstacle in the advancement of machine learning given it is a time-consuming and challenging process, requiring a considerable level of domain expertise~\cite{zoph2016neural}. In current literature, ANN structures are typically chosen based on their reputation or based on knowledge shared across the machine learning community. However, changing even a few problem-specific meta-parameters can lead to poor generalization upon committing to a specific topology~\cite{erkaymaz2014impact,Barna1990}.  To address these challenges, a number of neural architecture search (NAS)~\cite{elsken2018neural,liu2018darts,pham2018efficient,xie2018snas,luo2018neural,zoph2016neural} and neuroevolution (NE)~\cite{stanley2019designing,darwish2020survey} methods have been developed to automate the process of ANN design. Recently, nature-inspired neural architecture search (NI-NAS) algorithms have shown increasing promise, including the Artificial Bee Colony (ABC)~\cite{horng2017fine},  Bat~\cite{yang2010new}, Firefly~\cite{yang2010nature}, and Cuckoo Search~\cite{leke2017deep} algorithms.

Ant colony optimization (ACO)~\cite{dorigo1996ant} is a particularly successful NI-NAS strategy that has been shown to be quite powerful when automating the design of recurrent neural networks (RNNs). Originally, ACO for NAS was limited to small structures based on Jordan and Elman RNNs~\cite{desell2015evolving} or was used as a process for reducing the number of network inputs~\cite{mavrovouniotis2013evolving}. Later work proposed generalizations of ACO for optimizing the synaptic connections within RNN memory cell structures~\cite{elsaid2018optimizing} and even entire RNN architectures within an algorithmic framework called Ant-based Neural Topology Search (ANTS)~\cite{elsaid2020ant}. In the ANTS process, ants traverse a single massively-connected ``superstructure'', searching for optimal RNN sub-networks which involves connectivity between RNN nodes both in terms of structure, \ie, all possible feed forward connections, and in time, \ie, all possible recurrent synapses that span many different time delays. This approach shares similarity to NAS methods in ANN cell and architecture design~\cite{liu2018darts,pham2018efficient,xie2018snas,cai2018proxylessnas,
%single/few shot methods%
guo2020single,bender2018understanding,dong2019one,zhao2020few}, which operate within a limited search space, generating cells or architectures with a pre-determined maximum number of nodes and edges~\cite{elsken2018neural}.

Most NE methods, instead of operating within fixed bounds, are constructive, continually adding and removing nodes/edges during the evolutionary process (\eg, NEAT~\cite{stanley2002evolving}, CoDeepNEAT~\cite{miikkulainen2019evolving} and EXAMM~\cite{ororbia2019examm}). Other strategies involve generative encoding, such as HyperNEAT~\cite{stanley2009hypercube}, where a generative system is evolved, which can then be used to create architectures as well as assign values to their synaptic weights. Nevertheless, these approaches still require manually specifying or constraining the size or scale of the generated architecture in terms of the number of layers and nodes. 

In general, constructive NAS methods often suffer from getting stuck in (early/poor) local minima or take considerable computation time to evolve structures that are sufficiently large in order to effectively address the task at hand, especially for large-scale machine learning problems. Alternatively, having to pre-specify bounds for the space of possible NAS-selected architectures often requires domain expertise and can lead to poorly performing or suboptimal networks if the bounds are incorrect, often  requiring many runs of varying bound values. In order to address these challenges, this work introduces a novel ACO-inspired algorithm, the \emph{BackPropagation-Free Continuous Ant-based Neural Topology Search} (BP-Free CANTS) procedure, utilizing a continuous search domain that flexibly facilitates the design of ANNs of any size. Synthetic continuous ant (\emph{cant}) agents move through this search space based on the density and distribution of pheromone signals, which emulates how ants swarm in the real world, and the paths resulting from their exploration are used to construct RNN architectures. BP-Free CANTS (as well as the original CANTS algorithm~\cite{elsaid2021continuous}, which we will call BP-CANTS in this work for clarity) is a distributed, asynchronous algorithm, which facilitates scalable usage of high performance computing (HPC) resources, and also utilizes communal intelligence to reduce the amount of training required for candidate evolved networks. Notably, the procedure allows for the selection of recurrent nodes from a suite of simple neurons and complex memory cells used in modern RNNs: $\Delta$-RNN units~\cite{ororbia2017diff}, GRUs~\cite{chung2014empirical}, LSTMs~\cite{hochreiter1997long}, MGUs~\cite{zhou2016minimal}, and UGRNNs~\cite{collins2016capacity}. 
% $\Delta$-RNN units~\cite{ororbia2017diff}, gated recurrent units (GRUs)~\cite{chung2014empirical}, long short-term memory cells (LSTMs)~\cite{hochreiter1997long}, minimal gated units (MGUs)~\cite{zhou2016minimal}, and update-gate RNN cells (UGRNNs)~\cite{collins2016capacity}. 

BP-Free CANTS is compared to state-of-the-art benchmark algorithms used in designing RNNs for time series data prediction: ANTS~\cite{elsaid2020ant} and BP-CANTS~\cite{elsaid2021continuous}.  In addition to eliminating the requirement for pre-specified architecture bounds, our BP-Free CANTS is shown to yield results that improve upon ANTS and BP-CANTS at a significantly lower computational cost.  
%or are competitive to ANTS and EXAMM 
%while reducing the number of user specified hyperparameters from $16$ in both EXAMM and ANTS down to $8$ in CANTS. 
Our BP-Free CANTS procedure also provides advancement to the field of NI-NAS in that it is able to efficiently select for high performing architectures while at the same time finding well performing weights \emph{without backpropagation}. While ACO has been applied to continuous domain problems before~\cite{socha2008ant,kuhn2002ant,xiao2011hybrid,gupta2014transistor,bilchev1995ant}, to the authors' knowledge, BP and BP-FREE CANTS are one of the first to simulate and apply the movements of ants through a continuous space to design unbounded graph structures and BP-Free CANTS is the first to simultaneously use ACO to determine network weights and architecture. 
BP-Free CANTS has the capacity to optimize the neural topology and the neural synaptic parameters without applying the time consuming backpropagation and gradient-descent process required for memetic algorithms such as CANTS or other NE-based methods, further reducing required computational power and time consumption. BP-FREE CANTS also provides means for its cants agents to evolve during the optimization process, which enhances the chances of reaching better performing models, while requiring fewer hyperparameters that are associated with cants' behavior. 


\begin{comment}
Hyperparameters:
EXAMM:
    population size
    number islands
    recurrent depth
    more fit crossover
    less fit crossover
    clone rate
    add edge rate
    add recurrent edge rate
    enable edge rate
    disable edge rate
    split edge rate
    add node rate
    enable node rate
    disable node rate
    split node rate
    merge node rate


ANTS:
    Max lag
    Number of hidden layers
    Number of hidden layer nodes
    Number of ants
    use_forward_social_ants (boolean)
    use_backward_social_ants (boolean)
    use_L1_pheromone_regularization (boolean)
    L1_parameter ([0,1])
    use_L2_pheromone_regularization (boolean)
    L2_parameter ([0,1])
    pheromone update constant (if not using regularization)
    use_jumping_ants (boolean)
    use_commual_weights_pooling_with_const_parameter (boolean)
            commual_weights_pooling_with_const_parameter ([0,1])
    use_commual_weights_pooling_with_fitness_function (boolean)
    pheromone_evaporation_parameter ([0,1])

CANTS:
	Max lag
	Number of ants
	Ants sensing radii
	Ants exploration instinct (to create new points rather than following pheromone when doing a step)
	DBSCAN max distance
	DBSCAN min number of points in a cluster
	Pheromone decay constant
	pheromone update constant
\end{comment}






%Recurrent neural networks (RNNs) have emerged as a transformative method for modeling cyber-physical systems (CPS), as they are capable of handling long term dependencies through modern memory cell architectures~\cite{ororbia2017diff,chung2014empirical,hochreiter1997long,zhou2016minimal,collins2016capacity} and they can effectively utilize CPS sensor data which consists of multiple non-seasonal, non-stationary time series streams correlated cross varying amounts of time; data which is hard to model with the traditional family of ARIMA statistical models.  However, the problem of determining optimal architectures, especially where optimality can vary in terms of RNN accuracy, performance, as well as memory and energy utilization from task to task, remains an open problem.


==> sections/91-revision-00.tex <==
\section*{Revision Responses}


\subsection{Reviewer 1}

\begin{enumerate}
    \item \textbf{\color{red} The abstract does not include numerical results to show the contribution of this work.}\\
    % \todo{ADD TABLE WITH NUMERIC VALUES}\\
    \respond{The abstract has been updated to include the following statement: \\
    ``Adding this extra dimension allows CANTS agents to optimize both the architecture as well as the weights of an ANN without applying backpropagation of errors (BP), which leads to a significant reduction in the time consumed with respect to the optimization process: at least an average of $96$\% less time consumption with competitive, if not better, optimization performance.``\\
    Also, tables containing numeric measurements have been added to the Results section (Section~\ref{sec:results}) in order to highlight and quantify the core contribution of the work.
    }
    
    \item \textbf{\color{red} The details of the recurrent neural network method are not clear in the explanation of the methodology section.}\\
    \respond{Additional details about the generation of recurrent neural networks in ANTS, BP-CANT, and BP-Free CANTS have been described in a previous publication. These details were omitted from this manuscript for editorial reasons. However, the previous publication is repeatedly referred to in the paper. For example, in the Methodology section:  ``Figure~\ref{fig:cants_move} shows scenarios of cants movement through the search space starting from an input to an output. The shown movements illustrate cants exploration of new spots in the search space, cants exploitation of previously searched areas, attracted by previous pheromone deposits, and how cant-paths are translated into a final candidate architecture (refer to~\cite{elsaid2021continuous} for more details).''}
    
    \item \textbf{\color{red} Could the proposed method be applied to different datasets?}
    \respond{Just like BP-CANTS (the backprobagation-centric version of the new method), BP-Free CANTS is very much applicable to any data that recurrent neural networks are applicable to. The computational system generates recurrent neural networks and is agnostic to the input data type (it is only required that the input is a multi-dimensional tensor). In previously published work~\cite{elsaid2021continuous}, BP-CANTS was applied to three different time series datasets, obtained from three different sources, belonging to two different industries - coal-fired power plants and wind-power generation. The fact that BP-Free CANTS extends the 3D search space of BP-CANTS to include a $4^{th}$ dimension extends the capacity of the method without limiting/hindering its current capabilities.}
    
    \item \textbf{\color{red} What is the computational complexity of the proposed method?}\\
    % \todo{HOW TO QUANTIFY THAT!}
    \respond{Thanks for advising about adding the complexity of the algorithms. A new paragraph has been added to the Methodology section (Section ~\ref{sec:method}) to address this key point:
        \input{sections/002.method_time_comlexity}
    }
    
    \item \textbf{\color{red} It is recommended to add some metrics to measure the proposed method's test performance.}\\
    \respond{Thank you for the feedback! 
        Figure~\ref{fig:time_accum} and the following paragraph were added under the Results sections to address this point:\\
        Figure~\ref{fig:time_accum} illustrates the time consumption-difference of BP-Free CANTS and BP-CANTS. The two methods were allowed to generate $200$ neural structures using $8$ CPUs and $35$ agents. The figures show the time consumed in order to generate the neural structure(s) where the two methods result in timings that were very close with BP-Free CANTS taking a bit more time to process the extra $4^{th}$ dimension. Observably, the evaluation time of BP-CANTS was an order of magnitude higher than that of the BP-Free CANTS because the former used BP, while the latter does not. The figure also shows the accumulative time of neural-structure-generation and the RNN-evaluation of the two methods as the iterations progress. The great difference between the cumulative time of BP-CANTS and BP-Free originates from the time consumed by BP. The slope of the cumulative time is higher at the early iterations compared to later ones because the search space is fairly empty/sparse (no pheromone deposits) in the beginning iterations, but as the number of iterations increases, the search space is gradually filled causing the agents to create more neurons, which increases the evaluation time. The curves then saturate a bit because of the pheromone-evaporation effect, which maintains the pheromone traces at about a constant level.
    }
    
    \item \textbf{\color{red} On page 2, please revise ``In the ANTS process, ants traverse a single massively connected "superstructure", searching for optimal RNN sub-networks which involves connectivity between RNN nodes both in terms of structure, i.e., all possible feed forward connections, and in time, i.e., all possible recurrent synapses that span many different time delays.''}
    \respond{Thank you for the note. The statement has been reviewed and we now alternatively use the statement: 
    ``ANTS utilizes a massively connected neural structure as a discrete structural search space. Although the approach has shown success, the main critique for the strategy is the limitation of discreteness of the search space.''}
    
    \item \textbf{\color{red} Please find some corrections as follows:}
    \begin{itemize}
        \item  \textbf{\color{red} On page 2, " Our BP-Free CANTS procedure also provides an advancement to the field of NI-NAS is that it is able to efficiently both select for high performing architectures while at the same time finding well performing weights without backpropagation. " might be written as " Our BP-Free CANTS procedure also provides advancement to the field of NI-NAS in that it is able to efficiently select for high performing architectures while at the same time finding well performing weights without backpropagation. "}
        \respond{Thank you for the recommendation. The statement has now been reworded based the reviewer suggestion.}
        
        \item \textbf{\color{red} On page 13, ``This work compares BP-Free CANTS to the previous state-of-the-art ANTS and BP-CANTS algorithmss on three real world datasets related to power systems. " might be written as " This work compares BP-Free CANTS to the previous state-of-the-art ANTS and BP-CANTS algorithms on three real world datasets related to power systems.''}
        \respond{Thank you for the recommendation -- the statement has been reworded accordingly based this suggestion.}
    \end{itemize}
\end{enumerate}

==> sections/92-revision-00.tex <==
\subsection{Reviewer 2}
    \begin{enumerate}
        \item \textbf{\color{red} In the highlight, CANTS can be scaled up. But in the RNN experiment, it took a total 2304 cores and 24 TB of RAM approximately 4 weeks. It seems contradictory. If authors could clarify more about the predicted time or resource in the scale up or CO2 emission, it would be great.}
        \respond{Thank you for the feedback. The Highlights section does not mention that the method uses this amount of computational power and memory. Those desired numbers were actually mentioned in the Results section under the subsection: \textit{Computing Environment}. Those measurements are specific to the total capacity of the computer cluster on which the experiments were scheduled but they are not the actual numbers representing the computing resources that were used to perform the experiments. Under the same sub-section, we mentioned that the experiments only used three nodes on the cluster, each has 36 cores, which means a total of 108 cores. It is also worth pointing out that the consumed computing time and resources were for all of the experiments performed, which was meant to be as comprehensive as possible to cover the important variability in the methods' features and parameters. However, more or less resources can definitely be used to only carry out the optimization task for a specific problem. Moreover, and more importantly, increasing the amount of used computational resources will decrease the time consumed because the resources are used to apply \emph{asynchronous distributed computation} which will thus scale up the computation performance.
        }
        
        \item \textbf{\color{red} Besides Ant colony optimization (ACO), other methods introduced in the introduction, such as Artificial Bee Colony (ABC) [11], Bat [12], Firefly [13], and Cuckoo Search [14] algorithms are also good in the evolutionary perspective. There is not a enough part to discuss why choose special ACO not other evolutionary algorithms.}
        \respond{Thank you for this important note. The reason behind choosing ACO was explicitly stated in published related work but was omitted from this manuscript for editorial reasons. However, paragraph 2 in the  ``Introduction'' has now been modified to justify using ACO:
        ``Ant colony optimization (ACO) - originally introduced as a graph optimization method~\cite{dorigo1996ant} - has proven itself to be a successful NI-NAS strategy. The reason ACO operates as a strongly feasible NAS method is rooted in the concept of its application as a graph optimization method, providing impressive results~\cite{manfrin2006parallel,bianchi2002ant,dorigo1997ant,dorigo1997ant_,dorigo1996ant,dorigo1992optimization,dorigo2006ant,peake2019scaling}. As the structure of neural networks themselves are in essence directed graphs, this makes ACO well-suited towards the problem of NAS.''
        }
        
        \item \textbf{\color{red} What is the difference between ACO and particle filtering or sequential Monte Carlo methods, as they are all based on some metrics to update the next time samples to align with the real state better?}
        \respond{
            % \begin{itemize}
            %     \item more expensive? $\rightarrow$ more evaluations each the Mont Carlo samples should cover the search space.
            %     \item how to map the neural space to the search space? $\rightarrow$ space is huge $\rightarrow$ too much computation in each iteration
            % \end{itemize}
            On the one hand, the main challenge that might face the application of a Monte Carlo-based methods like particle filter might be the mapping of the neural architecture search (NAS) space into the method's search space. On the other hand, ACO was originally introduced as a successful graph-optimization algorithm, making the adoption of ACO for a graph-based optimization problems, like neural structure optimization, effective and efficient. Moreover, particle filtering is computationally expensive, especially when working on massive search spaces like in the NAS realm. Particle filtering is susceptible to `particle impoverishment`, a problem effecting the efficacy of the method when sampling the particles, which is exacerbated when working on vast (high-dimensional/large) search spaces. Interestingly enough, there is published research work that has investigated the application of ACO to solve the particle filtering particle-impoverishment problem~\cite{heris2014ant,zhong2010biologically}
        }
        \item \textbf{\color{red} Hinton recently proposed the forward-forward algorithm, which abandons end-to-end layer backpropagation and shows good performance in some tasks. How would the authors compare it with forward-forward?}
        \respond{Hinton's forward-forward algorithm for adapting neural synpatic parameters is indeed very interesting but it is (quoting from Hinton's article) "\ul{slower} than backpropagation and does not generalize quite as well on several of the toy problems investigated"~\cite{hinton2022forward}. In this introduced work, we are not claiming absolute superiority over the performance of backpropagation, as we observe BP performance to remain robust, albeit slow. The main advantage of our method over BP is that it not only optimizes the neural parameters (synaptic weights), but it also optimizes the neural structure, offering a neuroevolution solution for the neural optimization problem, doing that in significantly less time than BP, and thus, - according to Hinton's article - faster than Hinton's forward-forward.\\ \\
        Another important point to note is that the forward-forward algorithm, as well as its cousin algorithm developed in parallel at the time, the predictive forward-forward algorithm, require a negative data generating process to be effective (which is particularly difficult to design for unsupervised sequence modeling tasks, as these two algorithms exploit the clean labels provided in classification benchmarks to craft ``wrong labels''). Our approach does not require the user to carefully design an effective contrastive process and its required negative data generative process and instead operates directly within the neural forward inference framework - in other words, one could call BP-Free CANTS as a forward-only, multi-agent optimization algorithm. Finally, forward-forward and predictive forward-forward learning only offer potential layer-wise parallelism (in the learning process) while BP-Free CANTS offers massive parallelism in terms of the individual agent optimization pathways.
        }
    \end{enumerate}

==> sections/93-revsion-00.tex <==
\subsection{Reviewer 3}
    \begin{enumerate}
        \item \textbf{\color{red} Please add the complexity of your algorithm}
        \respond{Thanks for advising about adding the complexity of the algorithms. A new paragraph is added in Section~\ref{sec:method} to address this point:
        ``\paragraph{Time Complexity of the Algorithms:} While the time complexity of the various ANTS algorithms is important, it should be noted that the time spent generating recurrent neural networks with these algorithms is orders of magnitude less than the time required to evaluate the fitness of the neural networks (which requires training and validation for ANTS and BP-CANTS and only validation for BP-Free CANTS). This is highlighted in Figure~\ref{fig:time_accum}. 
        For ANTS and BP-CANTS, each generated recurrent neural network (which may have tens of thousands of trainable parameters) needs to be trained using backpropagation through time (BPTT) for a number of epochs. Given that all the ANTS algorithms use an asynchronous distributed/parallel execution strategy, training potentially hundreds of RNNs simultaneously on distributed compute nodes while the master process, which generates new RNNs, spends most of its time waiting for more work requests from the workers (it may take fractions of a second to generate a network, however, training them and then evaluating them on the validation dataset can take multiple minutes, even for the few number of epochs required). For BP-Free CANTS, even the forward pass of the network over the validation data to evaluate the network without BP is still orders of magnitude faster than the time required for the algorithm to generate the networks.\\
        That being said, the time complexity of these algorithms (in terms of network generation) is O(N log N) where N is the number of pheromones deposited when the ants traverse the search space, due to utilizing DBSCAN to cluster these points in space -- DBSCAN can be done in O(N log N) using an optimized version. The number of pheromones deposited is a factor of the number of cants $A$ and the smallest movement range (0.1) that a cant will move forward. As the farthest distance in the graph is $1.0$, this means each cant can deposit at most $10$ pheromones (and thus $10$ edges, as edges are generated when ants move between pheromones).  All other aspects of the algorithms (i.e., network construction) take O(C) time, which is the number of clusters produced by DBSCAN. The maximum number of clusters is $10 * A$, assuming that all ants produce pheromones which do not cluster. Therefore, the time complexity of CANTS and BP-CANTS is O(A log A) where A is the number of cants, as the complexity is dominated by utilizing DBSCAN.''
    }
        
        \item \textbf{\color{red} Please add a discussion section after the results section or along with the results in the form of results and discussion, in this work section, please compare your work and your proposed model with other models, discuss the advantages and disadvantages, and use valid articles to prove your reasoning and the accuracy of your proposed model.}\\
        \respond{The advantages of our new method -- BP-Free CANTS -- are stated in the Results sections, and summarized in the Discussion and Future Work Section: ``Our results demonstrate that BP-Free CANTS improves over ANTS and BP-CANTS while running substantially and significantly faster'', and ``BP-Free CANTS can provide a well performing solution to the design and training of networks which have activation functions or other components for which derivatives cannot be calculated (which preclude them from utilizing backpropagation), such as models with sampled activities (e.g., Bernoulli distribution) or even discrete ones such as spiking neural networks.''
        \\
        For the disadvantages, this statement is added to the Discussion and Future Work section: ``A potential disadvantage of BP-Free CANTS is that if enough computational resources are available to offer BP-based NAS methods a significant number of training epochs (without worry about cost or emissions), the accuracy of the resulting models will be higher than of BP-Free Cants. Nevertheless, the computational cost of BP is always a burden in NAS methods, and a good reason to seek faster alternatives"~\cite{miller1990cmac,1007668,406684,ORKCU20113703}.}
        
        % \todo{refer to comparisons made in previous CANTS publication and build on that to conclude that if BP-Free CANTS is getting those good results against BP-CANTS and ANTS, and BP-CANTS and ANTS did well against NEAT and EXAMM while using the same dataset, then BP-Free CANTS results are novel contribution}\\
        
        \item \textbf{\color{red} Which equation is newly proposed in the paper?}
        \respond{The formal notation and equations representing the novel contribution of this work are: 
        \begin{itemize}
            \item The equation used for the cants movement through the search space:
            \[
                sense\_range_{precieved} =  max \Big( sense\_radius - \big( y^2 \times r_1 + y \times r_2 \big), 0.1 \Big)
            \]
            \item Also, the cants evolution algorithm ($cant.evolve()$), which utilizes a genetic algorithm to evolve the optimization agents behavior, is one of the central contributions of this work. 
        \end{itemize}
        }
        
        \item \textbf{\color{red} How do you argue that this method works in different optimization processes in the field of applications?}
        \respond{Manually optimizing ANN structures has been an obstacle to the advancement of machine learning as it consumes significant amount of time and requires a considerable level of experience in the domain~\cite{zoph2016neural}. Due to the ever increasing sizes of ANN models designed to meet the demand of the ever increasing complexity of data science and machine learning problems, NAS and neuro-evolution (NE) have become a logical next step towards the automation of ANN design~\cite{elsken2018neural}. The method that this work has introduced for neural architectural search (NAS) and neuro-evolution (NE) applications and was compared to the benchmark and state-of-the-art in the field: NEAT, EXAMM - in previous publications -, and ANTS, using real world datasets obtained from different disciplines.}
    \end{enumerate}
